AS Relationships: Inference and Validation

Research on performance, robustness, and evolution of the global Internet is fundamentally handicapped without accurate and thorough knowledge of the nature and structure of the contractual relationships between Autonomous Systems (ASs). In this work we introduce novel heuristics for inferring AS relationships. Our heuristics improve upon previous works in several technical aspects, which we outline in detail and demonstrate with several examples. Seeking to increase the value and reliability of our inference results, we then focus on validation of inferred AS relationships. We perform a survey with ASs' network administrators to collect information on the actual connectivity and policies of the surveyed ASs. Based on the survey results, we find that our new AS relationship inference techniques achieve high levels of accuracy: we correctly infer 96.5% customer to provider (c2p), 82.8% peer to peer (p2p), and 90.3% sibling to sibling (s2s) relationships. We then cross-compare the reported AS connectivity with the AS connectivity data contained in BGP tables. We find that BGP tables miss up to 86.2% of the true adjacencies of the surveyed ASs. The majority of the missing links are of the p2p type, which highlights the limitations of present measuring techniques to capture links of this type. Finally, to make our results easily accessible and practically useful for the community, we open an AS relationship repository where we archive, on a weekly basis, and make publicly available the complete Internet AS-level topology annotated with AS relationship information for every pair of AS neighbors.

==> Makefile <==
ROOT=as_rel

TEXSRC=	$(ROOT).tex $(ROOT).bbl

all: $(ROOT).pdf

.SUFFIXES: .tex .dvi .ps .pdf .obj .eps

$(ROOT).dvi: $(TEXSRC)

MKPASS=@mkpass() { rm -f $(ROOT).dvi; $(MAKE) $(ROOT).dvi && touch $$*;}; mkpass

.pass1: $(TEXSRC) $(IMAGES)
	$(MKPASS) $@

.pass2: .pass1
	$(MKPASS) $@

$(ROOT).ps: .pass2

.tex.dvi:
	latex \\nonstopmode \\input{$<} || { rm $@; exit 1; }

.dvi.ps:
	dvips -t letter -Ppdf -G0 -o $@ $<

.ps.pdf:
	ps2pdf -dCompatibilityLevel=1.3 $<

.ps.eps:
	convert $< $@

.obj.eps:
	@rm -f $@
	@TMPDIR=$${TMPDIR:-/tmp} tgif -print -eps $<

.ps.png:
	gs -q -dNOPAUSE -dBATCH -sDEVICE=png256 -sOutputFile=$@ -c save pop -f $<

clean:
	rm -f *.aux *.log *~
	rm -f .pass[123] .rebuild

realclean: clean
	rm -f *.ps *.dvi *.pdf *.sav *.bak
	chmod -x `find . -type f`

